Scaling behavior of discretization errors in renormalization and improvement constants

Non-perturbative results for improvement and renormalization constants needed for on-shell and off-shell O(a) improvement of bilinear operators composed of Wilson fermions are presented. The calculations have been done in the quenched approximation at beta=6.0, 6.2 and 6.4. To quantify residual discretization errors we compare our data with results from other non-perturbative calculations and with one-loop perturbation theory.

==> Makefile <==
# %auto-ignore
GIF_SRC = 
PNG_SRC = 
JPG_SRC = 
EPS_SRC = 
FIG_SRC = 
TEX_SRC = tab2pt3pt tabmtilde tabfinalNP tabcprimeNP tab_cV tab_cp_comp
AX_SRC = kappac c_A_tuning64 cAext60f cAext62 cAext64 Zvslope ZV_sub23 Zvbvba Zvbvba_m1 \
	   cVfit cVfit1 cVfit2 cVND cVpolefit \
           ZAcomp ZVZAZA ZAfitm ZPZS ZPZSfit cT2 cT3 cTvsm cprime \
           cA62vspa2pt_3pt cA64vspa2pt_3pt
#          bPbA cAext60b cVfit3 ZVplot
OTHER_SRC = 
MAIN = paper

${MAIN}.pdf: ${GIF_SRC:%=%.png} ${PNG_SRC:%=%.png} \
             ${JPG_SRC:%=%.jpg} ${EPS_SRC:%=%.pdf} \
             ${FIG_SRC:%=%.pdf} ${TEX_SRC:%=%.tex} \
             ${AX_SRC:%=%.pdf} ${MAIN}.tex

SOURCES=${GIF_SRC:%=%.gif} ${PNG_SRC:%=%.png} \
            ${JPG_SRC:%=%.jpg} ${EPS_SRC:%=%.eps} \
            ${FIG_SRC:%=%.fig} ${TEX_SRC:%=%.tex} \
            ${AX_SRC:%=%.ax} \
            ${MAIN}.tex Makefile ${OTHER_SRC}

src.tar.gz: ${SOURCES}
	tar cvfz $@ $^

PSINCLUSIONS= ${AX_SRC:%=%.ps} ${FIG_SRC:%=%.ps} ${EPS_SRC:%=%.eps}

.SUFFIXES: .gif .png .jpg .eps .pdf .fig .tex .ax

%.pdf: %.tex
	rm -f thumb[0-9][0-9][0-9].png
	pdflatex $< && bibtex $* && pdflatex $< && pdflatex $<
	while [ `grep '^Rerun ' $*.log` ]; do pdflatex $<; done
	rm -f thumb[0-9][0-9][0-9].png

%.eps: %.fig
	fig2dev -L ps < $< > $@

# ghostscript (incomplete)
%.pdf: %.eps
	epstopdf $<
%.pdf: %.ps
	epstopdf $<
%.pnm: %.eps
	pstopnm $< > $@

%.png: %.pnm
	pnmtopng $< > $@
%.pnm: %.gif
	giftopnm $< > $@


# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@.tmp
	sed -e "s/%%BoundingBox: (atend)/`psbbox $@.tmp | head -1`/p" \
            -e '/%%BoundingBox/d' $@.tmp > $@ 
	rm -f $@.tmp
%.ps: %.xy
	xyplot $< | epsplot > $@.tmp
	sed -e "s/%%BoundingBox: (atend)/`psbbox $@.tmp | head -1`/p" \
            -e '/%%BoundingBox/d' $@.tmp > $@ 
	rm -f $@.tmp

# else look for a dvi file.
%.ps: %.dvi
	dvips  $< -o
%.dvi: %.tex
	latex $< && bibtex $* && latex $< && latex $<
	-while [ `grep '^Rerun ' $*.log` ]; do latex $< ; done

# Save paper
%.ps2: %.ps
	pstops -w21cm -h29.7cm '2:0L@.65(1w,0)+1L@.65(1w,.45h)' $< | sed -e '1a\
	%%Orientation: Landscape' > $@

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS} ${MAIN:%=%.bbl} ${MAIN:%=%.bib}
	rm -f submission.uu
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS} ${MAIN:%=%.bbl} ${MAIN:%=%.bib}" ; \
	 echo "submission") | uufiles -gz -9


